AutoPatch: Automated Generation of Hotpatches for Real-Time Embedded Devices

Real-time embedded devices like medical or industrial devices are increasingly targeted by cyber-attacks. Prompt patching is crucial to mitigate the serious consequences of such attacks on these devices. Hotpatching is an approach to apply a patch to mission-critical embedded devices without rebooting them. However, existing hotpatching approaches require developers to manually write the hotpatch for target systems, which is time-consuming and error-prone. To address these issues, we propose AutoPatch, a new hotpatching technique that automatically generates functionally equivalent hotpatches via static analysis of the official patches. AutoPatch introduces a new software triggering approach that supports diverse embedded devices, and preserves the functionality of the official patch. In contrast to prior work, AutoPatch does not rely on hardware support for triggering patches, or on executing patches in specialized virtual machines. We implemented AutoPatch using the LLVM compiler, and evaluated its efficiency, effectiveness and generality using 62 real CVEs on four embedded devices with different specifications and architectures running popular RTOSes. We found that AutoPatch can fix more than 90% of CVEs, and resolve the vulnerability successfully. The results revealed an average total delay of less than 12.7 $\mu s$ for fixing the vulnerabilities, representing a performance improvement of 50% over RapidPatch, a state-of-the-art approach. Further, our memory overhead, on average, was slightly lower than theirs (23%). Finally, AutoPatch was able to generate hotpatches for all four devices without any modifications.

==> Sections/ACAlgorithmA.tex <==
\section{AC Algorithm}

Algorithm~\ref{alg_ana} describes the workflow of AC. 
In the first step (Lines 2-8), AC finds the best trampoline based on whether the official patch is in the branch or not, 
and then stores the instructions between the selected trampoline and the patch in $AInsts$ using the $identifyInstructions()$.
It should be noted that AC receives as input the location of the official patch in the vulnerable function from the RTOS developer.
Afterwards (Lines 9-13), AC starts analyzing backwards from the last instruction in $AInsts$, which is the instruction above the patch location ($pLocation$).
If the instruction ($Ainst_i$) modifies a variable of the patch, 
AC replaces that variable with the value on the right side of the instruction; otherwise, AC skips it.
AC continues this analysis until it reaches the selected trampoline (i.e., best trampoline).
Once the trampoline is reached, AC stores the obtained instructions ($PInsts$) in $HInsts$ (Line 14). 
In the future steps (discussed in Section~\ref{patchasec}), these instructions ($HInsts$) form the hotpatch that will be executed by the selected trampoline.


\begin{algorithm}[h]
	\caption{Analysis Component Algorithm}	\label{alg_ana}
	\SetKwInOut{Input}{inputs}
	\SetKwInOut{Output}{output}
	\SetKwProg{analysisComponent}{analysisComponent}{}{}
	
	\analysisComponent{$()$}{
		\Input{Vulnerable Function ($Insts = inst_{1} \dots inst_{n}$)\newline Official Patch ($PInsts = pinst_{1} \dots pinst_{n}$)\newline  Patch Location ($pLocation$) \newline
		List of Trampolines ($Tramps = t_{1} \dots t_{n}$)}
		\Output{Hotpatch ($HInsts = hinst_{1} \dots hinst_{n}$)}

		\uIf {$PInsts$ inside a $branch$}{
			\eIf{$branch.depth()  > 1$ || $branch.condition$ has a $pointer$}{
				$bestTrampoline := findTrampoline(Tramps)$; %\Comment{The closest to the patch and inside the branch}\newline
				$AInsts := identifyInsts(bestTrampoline,Insts,pLocation)$;
			}
			{ 	
				$bestTrampoline := findTrampoline(Tramps)$; %\Comment{The closest to the patch and outside the branch}\newline
				$AInsts := identifyInsts(bestTrampoline,Insts,pLocation)$;
			}
		}
		\Else {
			$bestTrampoline := findTrampoline(Tramps)$;
			$AInsts := identifyInsts(bestTrampoline,Insts,pLocation)$;
			
		}
		\ForEach{instruction $Ainst_i \in AInsts = Ainst_{n} \dots Ainst_{1} $}{ 
			
			\uIf{$Ainst_i$ changes a variable of $PInsts$}{
				$PInsts.variable$ <- $Ainst_i$;\newline
				\Comment{Replace the variable with value of $Ainst_i$}
			}
			\Else{
				continue;
			}
		}
		$HInsts := PInsts$ \;
	}
	\KwRet{$HInsts = hinst_{1} \dots hinst_{n}$}\;
\end{algorithm}


==> Sections/ICAlgorithmA.tex <==
\section{IC Algorithm}

Algorithm~\ref{alg_ins} demonstrates how IC iterates through each instruction (lines 6-25) and checks its type (lines 7, 15 and 18). 
If the instruction is found to be one of the instrumentation locations (e.g., lines 7-12), 
IC uses the $identifyLocation()$ to obtain the appropriate location for adding the trampoline. 
Once the location is identified, IC calls the $insertTrampoline(Location)$ to add the trampoline to that location.
Otherwise, if the instruction type is not one of the instrumentation locations (e.g., lines 13-14), IC skips it. 
The aforementioned operation is performed for each function in the application until reaching its end. 
Ultimately, the output of this process consists of the instrumented functions within the application.

\begin{algorithm}[h]
	\caption{Instrumentation Component Algorithm} 	\label{alg_ins}
	\SetKwInOut{Input}{inputs}
	\SetKwInOut{Output}{output}
	\SetKwProg{instrumentationComponent}{instrumentationComponent}{}{}
	\instrumentationComponent{$(Insts)$}{
		\Input{Function ($Insts = inst_{1} \dots inst_{n}$)}
		\Output{Instrumented Function}

		\uIf {Function Entrance}{
			$location := identifyLocation()$\;
			$insertTrampoline(location)$;
		}
		\Else {
			\ForEach{instruction $inst_i \in Insts$}{%
			
				\uIf{$inst_i.type$ is a $branch\_instruction$}{%
					\eIf{$branch.depth()  > 1$}{
						$beginL := identifyLocation(branch)$\;
						$endL := identifyLocation(branch)$\;
						$insertTrampoline(beginL)$\;
						$insertTrampoline(endL)$;
					}
					{ 	
						continue;
					}
				}
				\uElseIf{$inst_i.type$ is a $function\_call$}{
					$location := identifyLocation()$\;
					$insertTrampoline(location)$;
				}
				\uElseIf{$inst_i.type$ is a $loop$}{
					\eIf{$loop.depth()  > 1$}{
						$beginL := identifyLocation(branch)$\;
						$endL := identifyLocation(branch)$\;
						$insertTrampoline(beginL)$\;
						$insertTrampoline(endL)$;
					}
					{ 	
						continue;
					}
				}
			}
		}
		\KwRet{$instrumentedFunction$}\;
	}
\end{algorithm}


==> Sections/RelatedA.tex <==
\section{Related Work Summarization}



 %\karthik{Maybe this can be in the main body of the paper as we have space now.}
 %\mohsen{After changing the location of Algorithms, we have extra one page (13 pages)!}
We provide a summary of the state-of-the-art hotpatching methods across different types of devices, 
including Android, real-time embedded systems, and general-purpose devices in Table~\ref{tab:compare}. 
As we analyze each of the proposed 
approaches~\cite{niesler2021hera,he2022rapidpatch,chen2018instaguard,chen2017adaptive,arnold2009ksplice}, 
we identify limitations that render them unsuitable for use on embedded devices. 
%\karthik{Summarize the limitations in 1-2 sentences}
In brief, the identified limitations of these hotpatching methods
include hardware dependencies (e.g., FPB) for patch triggering, 
dependence on an additional programming language and VM to execute the patch, 
and runtime modifications of the program code, all of which render them impractical for use on 
real-time embedded devices.
To address these limitations and automatically generate patches for device vulnerabilities, 
we introduce \SN{}. %By doing so, we build upon previous work and provide an effective solution 
%that fixes the problems of earlier methods.

\definecolor{Gray}{gray}{0.9}
\newcolumntype{g}{>{\columncolor{Gray}}c}
\begin{table}[!ht]
  
  \begin{center}
   \caption{A subjective comparison between \SN{} and state-of-the-art hotpatching methods proposed
    for Android (A) devices, real-time Embedded (E) devices, and General Purpose (GP) devices. CCR and RP denote change code at runtime
    and rewrite patch in other language, respectively.}
   \label{tab:compare}
   \begin{tabular}{c|ccccc|g}
    Objectives & {\rotatebox[origin=c]{90}{ HERA \cite{niesler2021hera}}} & {\rotatebox[origin=c]{90}{RapidPatch \cite{he2022rapidpatch}}} & {\rotatebox[origin=c]{90}{ Instaguard \cite{chen2018instaguard}}}  & {\rotatebox[origin=c]{90}{ KARMA\cite{chen2017adaptive}}} & {\rotatebox[origin=c]{90}{ Ksplice \cite{arnold2009ksplice}}} & {\rotatebox[origin=c]{90}{ \SN{} }} \\ 
    \hline \hline
    Target& E& E & A & A & GP & E\\ 
    w/o Need Hardware& \xmark & \cmark & \xmark & \cmark & \cmark & \cmark\\
    w/o CCR& \cmark & \cmark & \cmark & \xmark & \xmark  & \cmark\\ 
    w/o Need VM& \cmark & \xmark & \cmark & \xmark & \cmark  & \cmark\\ 
    w/o RP& \cmark & \xmark & \xmark & \xmark & \cmark & \cmark\\ 
    Common Patch& \xmark & \cmark & \xmark & \cmark & \cmark  & \cmark\\ 

    \hline 
   \end{tabular}
  \end{center}
 \end{table}

==> Sections/ResultsSA.tex <==
\section{Evaluation Results}
\label{sec:evaluation-extra}

%mention the frequency of these two boards
%and the results are better (compare to nRF board as the baseline)
%also say again this shows the generality of AutoPatch without modification

Since \SN{} works on LLVM, it is a platform-agnostic technique. 
Therefore, it can generate hotpatches for various
boards with diverse specifications and architectures, requiring no modifications to its implementation.
To validate its generality, in addition to the nRF52840 board, 
whose results were analyzed in detail in Section~\ref{sec:eval-efficiency}, 
we also executed \SN{} for the STM32-F446RE\footnote{We set the board frequency to 96 MHz.} and ESP-WROOM32 boards (details in Table~\ref{tab:specification}). 
Results in Table~\ref{table-CVE-dataset-appendix}, including hotpatch execution and memory overhead, 
demonstrate \SN{}'s ability to generate hotpatches for the mentioned CVEs in Table~\ref{table-CVE-dataset} 
across these boards without implementation changes. 

As shown in Table~\ref{table-CVE-dataset-appendix}, several observations can be made:
(1) Overheads are lower for the latter two boards due to their higher frequency compared to nRF52840 
(Section~\ref{sec:eval-efficiency}). The overhead difference of each CVE between each board and nRF52840 is written in parentheses.
Hence, a higher overhead indicates a lesser improvement compared to the nRF52840 board.
(2) The overhead pattern of CVEs is nearly identical between the nRF52840 and STM32-F446RE boards, 
which have the same architecture but differ in specifications. 
For instance, CVE-2020-10023 and CVE-2018-16528 incur minimum and maximum overhead, respectively.
In contrast, the overhead pattern differs for the ESP-WROOM32 board, 
which has different architecture and specifications. 
For example, CVE-2020-10024 has the lowest overhead but similarly CVE-2018-16528 has the highest overhead.
(3) Even though the ESP-WROOM32 board operates at a higher frequency than the STM32-F446RE, 
it is essential to note that frequency alone does not affect overhead. 
Various factors, including architecture, contribute to this metric. 
As a result, the overhead of the ESP-WROOM32 is lower than that of the STM32-F446RE in some 
CVEs, while in other CVEs, it is higher.
%\mohsen{I am not sure about this.}
%\mohsen{What we should do for "distribution size" comment?}

%ADD distribution size of functions for instrumentation overhead in a graph.


% Although ESP-WROOM32 board frequency is higher than STM32-F446RE, 
% this is not the only factor that affects the overhead and it depends on other factors such as architecture. 
% Therefore, in some CVEs the overhead of ESP-WROOM32 is less and in some cases more than STM32-F446RE.


%say few observations based on the Table: (1) Both of them better than nrf since they have higher frequency.
%(2) min and max for both arm-based boards are similar : 10023 - 16528
%(3) but for ESP it is different and its minimum is 10024 but still the max is 16528.
%(4) the results between these two boards 



%Notably, overheads are lower for the latter two boards due to their higher frequency compared to nRF52840 (Section~\ref{sec:eval-efficiency}).
%\mohsen{But results for STM board is better than ESP board while ESP has higher frequency.}
% \SN{} was able to generate hotpatches for mentioned CVEs in Table~\ref{table-CVE-dataset} 
% for these boards without changing the implementation. 
% Furthermore, we measured their execution overhead, which is shown in Table~\ref{table-CVE-dataset-appendix}. 
% As can be seen in parentheses for each CVE, the overheads are lower compared to the nRF52840 board 
% since the frequency of these two boards is higher than the nRF52840 board.


\begin{table}
	\centering
	\caption{Execution time ($\mu s$) and memory overhead ($Bytes$) of \SN{} on STM32-F446RE and ESP-WROOM32 boards 
	for different CVE types (Table~\ref{table-CVE-dataset}). Hotpatch execution overhead percentage compared to nRF52840 board are written in parentheses for each CVE.}
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{c|c:c|c:c}
		& \multicolumn{2}{c|}{STM32-F446RE} & \multicolumn{2}{c}{ESP-WROOM32} \\
		\cline{2-3} \cline{4-5}
	CVE No.    &   \begin{tabular}[c]{@{}c@{}}Execution\\Time ($\mu s$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory\\Usage (Bytes)\end{tabular}  &   \begin{tabular}[c]{@{}c@{}}Execution\\Time ($\mu s$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory\\Usage (Bytes)\end{tabular}  \\ 
	\hline \hline
	2020-10021  &   0.21  (32.2\%)        &   528          &   0.19 (38.7\%) & 732\\
	2020-10023  &   0.12  (40\%)          &   504         &   0.19 (5\%) & 576\\
	2020-10024  &   0.15  (42.3\%)        &   392          &   0.14 (46.1\%) & 524\\
	2020-10028  &   0.23  (41\%)          &   400         &   0.26  (33.3\%) & 556\\
	2020-10062  &   0.33  (31.2\%)         &  780          &   0.33  (31.2\%) & 1280\\
	2020-10063  &   0.21  (41.6\%)          & 400          &   0.16  (55.5\%) & 732\\ 
	\hline
	2018-16524  &   0.25  (32.4\%)           &  548        &   0.31 (16.2\%) & 720\\
	2018-16528  &   0.24 + 0.27 (33.7\%)      & 468 + 476        &   0.37 + 0.35 (6.5\%) & 708 + 772 \\
	2018-16603  &   0.27  (34.1\%)             & 516      &   0.35  (14.6\%) & 744\\ 
	\hline 
	2017-2784   &   0.18  (30.7\%)              & 380      &   0.17 (19\%) & 488\\
	2020-17443  &   0.21  (32.2\%)              &  476     &   0.18 (41.9\%) & 648\\
	2020-17445  &   0.27  (34.1\%)               &  560    &   0.29 (29.2\%) & 864 \\                                            
		\hline
	\textbf{Average} & \textbf{0.24 (35.1\%)} & \textbf{535} & \textbf{0.27 (27.3\%)}  & \textbf{778.5}
\end{tabular}
	}
	\label{table-CVE-dataset-appendix}
\end{table}


% Without memory
% \begin{table}
% 	\centering
% 	\caption{Execution time ($\mu s$) of \SN{} on STM32-F446RE and ESP-WROOM32 boards 
% 	for different CVE types (Table~\ref{table-CVE-dataset}). Hotpatch execution overhead percentage compared to nRF52840 board are written in parentheses for each CVE.}
% 	\resizebox{\columnwidth}{!}{%
% 	\begin{tabular}{c|c|c}
		
            
% 	CVE No.    &   STM32-F446RE & ESP-WROOM32\\ 
% 	\hline \hline
% 	2020-10021  &   0.21  (32.2\%)                     &   0.19 (38.7\%) \\
% 	2020-10023  &   0.12  (40\%)                       &   0.19 (5\%) \\
% 	2020-10024  &   0.15  (42.3\%)                     &   0.14 (46.1\%) \\
% 	2020-10028  &   0.23  (41\%)                       &   0.26  (33.3\%) \\
% 	2020-10062  &   0.33  (31.2\%)                     &   0.33  (31.2\%)\\
% 	2020-10063  &   0.21  (41.6\%)                     &   0.16  (55.5\%)\\ 
% 	\hline
% 	2018-16524  &   0.25  (32.4\%)                     &   0.31 (16.2\%) \\
% 	2018-16528  &   0.24 + 0.27 (33.7\%)               &   0.37 + 0.35 (6.5\%) \\
% 	2018-16603  &   0.27  (34.1\%)                     &   0.35  (14.6\%)\\ 
% 	\hline
% 	2017-2784   &   0.18  (30.7\%)                     &   0.17 (19\%) \\
% 	2020-17443  &   0.21  (32.2\%)                     &   0.18 (41.9\%) \\
% 	2020-17445  &   0.27  (34.1\%)                     &   0.29 (29.2\%) \\                                            
% 		\hline
% 	\textbf{Average} & \textbf{0.24 (35.1\%)} & \textbf{0.27 (27.3\%)}  
% \end{tabular}
% 	}
% 	\label{table-CVE-dataset-appendix}
% \end{table}



% \begin{table}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% 	\begin{tabular}{c|c|c}
		
            
% 	CVE No.    &   STM32-F446RE & ESP-WROOM32\\ 
% 	\hline \hline
% 	2020-10021  &   0.38  (67\%)                     &   0.19 (83.4\%) \\
% 	2020-10023  &   0.31  (71.5\%)                    &   0.48 (56\%) \\
% 	2020-10024  &   0.40  (63.6\%)                     &   0.14 (87.2\%) \\
% 	2020-10028  &   0.48  (64.4\%)                     &   0.46  (65.9\%) \\
% 	2020-10062  &   0.80  (64.8\%)                     &   0.32  (85.8\%)\\
% 	2020-10063  &   0.40  (68.7\%)                     &   0.14  (89\%)\\ 
% 	\hline
% 	2018-16524  &   0.42  (67.7\%)                     &   0.47 (63.8\%) \\
% 	2018-16528  &   0.41 + 0.45 (66.8\%)               &   0.42 + 0.38 (69.1\%) \\
% 	2018-16603  &   0.42  (67.2\%)                     &   0.47  (63.2\%)\\ 
% 	\hline
% 	2017-2784   &   0.35  (68.7\%)                     &   0.16 (85.7\%) \\
% 	2020-17443  &   0.38  (66.6\%)                     &   0.18 (84.2\%) \\
% 	2020-17445  &   0.48  (66.2\%)                     &   0.47 (66.9\%) \\                                            
% 		\hline
% 	\textbf{Average} & \textbf{0.47 (66.9\%)} & \textbf{0.35 (75.3\%)}  
% \end{tabular}
% 	}
% 	\caption{Execution time ($\mu s$) of \SN{} on STM32-F446RE and ESP-WROOM32 boards 
% 	for different CVE types (Table~\ref{table-CVE-dataset}). Hotpatch execution overhead percentage compared to nRF52840 board are written in parentheses for each CVE.}
% 	\label{table-CVE-dataset-appendix}
% \end{table}

% \begin{table}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% 	\begin{tabular}{c|c:c|c:c}
% 		& \multicolumn{2}{c|}{STM32-F446RE} & \multicolumn{2}{c}{ESP-WROOM32} \\
%             \cline{2-3} \cline{4-5}
% 	CVE No.    &   \SN{} & RapidPatch  &   AutoPatch & RapidPatch  \\ 
% 	\hline \hline
% 	2020-10021  &   0.38            &   X   &   X            &   X  \\
% 	2020-10023  &   0.31            &   X   &   X            &   X  \\
% 	2020-10024  &   0.40            &   X   &   X            &   X  \\
% 	2020-10028  &   0.48            &   X   &   X            &   X  \\
% 	2020-10062  &   0.80            &   X   &   X            &   X  \\
% 	2020-10063  &   0.40            &   X   &   X            &   X  \\ 
% 	\hline
% 	2018-16524  &   0.42            &   X   &   X            &   X  \\
% 	2018-16528  &   0.41 + 0.45     &   X   &   X            &   X  \\
% 	2018-16603  &   0.42            &   X   &   X            &   X  \\ 
% 	\hline
% 	2017-2784   &   0.35            &   X   &   X            &   X  \\
% 	2020-17443  &   0.38            &   X   &   X            &   X  \\
% 	2020-17445  &   0.48            &   X   &   X            &   X  \\                                            
% 		\hline
% 	\textbf{Average} & \textbf{0.47} & \textbf{X}  & \textbf{X} & \textbf{X} 
% \end{tabular}
% 	}
% 	\caption{Execution time ($\mu s$) of \SN{} and RapidPatch on STM32-F446RE and ESP-WROOM32 boards for different CVE types (Table~\ref{table-CVE-dataset}).}
% 	\label{table-CVE-dataset-appendix}
% \end{table}


% \begin{table}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% 	\begin{tabular}{c|c:c|c:c}
% 		& \multicolumn{2}{c|}{STM32-F446RE} & \multicolumn{2}{c}{ESP-WROOM32} \\
%             \cline{2-3} \cline{4-5}
% 	CVE No.    &   \begin{tabular}[c]{@{}c@{}}Execution\\Time ($\mu s$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory\\Usage (Bytes)\end{tabular}  &   \begin{tabular}[c]{@{}c@{}}Execution\\Time ($\mu s$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory\\Usage (Bytes)\end{tabular}  \\ 
% 	\hline \hline
% 	2020-10021                                  &   1.15            &   1024         &   1.15            &   1024                                                                                                     \\
% 	2020-10023  &   1.15            &   1024   &   1.15            &   1024  \\
% 	2020-10024  &   1.15            &   1024   &   1.15            &   1024  \\
% 	2020-10028  &   1.15            &   1024   &   1.15            &   1024  \\
% 	2020-10062  &   1.15            &   1024   &   1.15            &   1024  \\
% 	2020-10063  &   1.15            &   1024   &   1.15            &   1024   \\ 
% 	\hline
% 	2018-16524  &   1.15            &   1024   &   1.15            &   1024    \\
% 	2018-16528  &   1.15            &   1024   &   1.15            &   1024  \\
% 	2018-16603  &   1.15            &   1024   &   1.15            &   1024  \\ 
% 	\hline
% 	2017-2784   &   1.15            &   1024   &   1.15            &   1024  \\
% 	2020-17443  &   1.15            &   1024   &   1.15            &   1024  \\
% 	2020-17445  &   1.15            &   1024   &   1.15            &   1024   \\                                            
% 		\hline
% 	\textbf{Average} & \textbf{1.42} & \textbf{953.3}  & \textbf{1.42} & \textbf{953.3} 
% \end{tabular}
% 	}
% 	\caption{Execution time ($\mu s$) of \SN{} and RapidPatch on STM32-F446RE and ESP-WROOM32 boards for different CVE types (Table~\ref{table-CVE-dataset}).}
% 	\label{table-CVE-dataset}
% \end{table}

